Rethinking Precision of Pseudo Label: Test-Time Adaptation via Complementary Learning

In this work, we propose a novel complementary learning approach to enhance test-time adaptation (TTA), which has been proven to exhibit good performance on testing data with distribution shifts such as corruptions. In test-time adaptation tasks, information from the source domain is typically unavailable and the model has to be optimized without supervision for test-time samples. Hence, usual methods assign labels for unannotated data with the prediction by a well-trained source model in an unsupervised learning framework. Previous studies have employed unsupervised objectives, such as the entropy of model predictions, as optimization targets to effectively learn features for test-time samples. However, the performance of the model is easily compromised by the quality of pseudo-labels, since inaccuracies in pseudo-labels introduce noise to the model. Therefore, we propose to leverage the "less probable categories" to decrease the risk of incorrect pseudo-labeling. The complementary label is introduced to designate these categories. We highlight that the risk function of complementary labels agrees with their Vanilla loss formula under the conventional true label distribution. Experiments show that the proposed learning algorithm achieves state-of-the-art performance on different datasets and experiment settings.

==> files/Abstract.tex <==
\section{Abstract}
Test-time adaptation (TTA) has been proven that exhibit good performance on testing data with different distributions. The main challenge of TTA is that neither the source domain data nor labels of the test-time samples are available, so the usual method is to represent the labels with the prediction of the trained source model in an unsupervised learning framework. Preview work such as 'tent' optimizes over unsupervised objectives such as the entropy of model predictions, effectively facilitating target feature learning. However, it's easily influenced by the quality of pseudo-labels, i.e., this method is constrained to some slightly shifted distribution. This work proposes a novel complementary learning strategy that takes advantage of the ``less probable categories'' to improve TTA. We highlight that the risk function of complementary labels agrees with their Vanilla loss formula with the ordinary actual distribution. Experiments show that the proposed learning algorithm achieves state-of-the-art performance on different datasets and experiment settings.
